Multiple injections of energetic electrons associated with the flare/CME event on 9 October 2021

We study the solar energetic particle (SEP) event observed on 9 October 2021, by multiple spacecraft including Solar Orbiter (SolO). The event was associated with an M1.6 flare, a coronal mass ejection (CME) and a shock wave. During the event, high-energy protons and electrons were recorded by multiple instruments located within a narrow longitudinal cone. An interesting aspect of the event was the multi-stage particle energization during the flare impulsive phase and also what appears to be a separate phase of electron acceleration detected at SolO after the flare maximum. We aim to investigate and identify the multiple sources of energetic electron acceleration. We utilize SEP electron observations from the Energetic Particle Detector (EPD) and hard X-ray (HXR) observations from the Spectrometer/Telescope for Imaging X-rays (STIX) on-board SolO, in combination with radio observations at a broad frequency range. We focus on establishing an association between the energetic electrons and the different HXR and radio emissions associated with the multiple acceleration episodes. We have found that the flare was able to accelerate electrons for at least 20 minutes during the nonthermal phase observed in the form of five discrete HXR pulses. We also show evidence that the shock wave has contributed to the electron acceleration during and after the impulsive flare phase. The detailed analysis of EPD electron data shows that there was a time difference in the release of low- and high-energy electrons, with the high-energy release delayed. Also, the observed electron anisotropy characteristics suggest different connectivity during the two phases of acceleration.

==> oldText.tex <==



% \begin{itemize}    
%     \item [\textbullet]
%     For the first time, observations of different phases of anisotropy during a single SEP event was possible. The thorough analysis of the intensity of the in-situ electrons observed by \textit{SolO} showed two different broken power-laws with different break energies and spectral indices. We found that the first broken power-law associated with the first component had a softer high energy channels compared to the high energy channels of the second broken power-law. The roll over of the power-laws were also at different energies prompting the existence of two separate acceleration mechanisms. 
% \end{itemize}

%This suggests that there may exist different acceleration processes on or near the Sun with different efficiencies. The acceleration mechanisms at the Sun responsible for the first in-situ component were efficient in accelerating electrons rapidly, but was not so efficient for high energy electrons. However, the acceleration mechanisms which correspond to the second in-situ component were efficient not only in accelerating low energy electrons but also high energy electrons as evident by the spectral index and roll over.

% \begin{itemize}    
%     \item [\textbullet]
%     We have found a clear physical separation in injection times for low and high energy electrons. We show that they correspond to different acceleration mechanisms observed at the Sun during this time. We have found that the low energy injection had good correspondence with the flare with a relative contribution from the shock wave. As for the injection of high energy electrons, we found that the shock wave was the main accelerator. This is primarily due to the presence of a broad tail of energetic electrons in the vicinity of the coronal shock wave during this time.  
% \end{itemize}

%The remote sensing observations in the X-ray, radio, EUV, and white light wavelengths suggest a complex relationship between the flare and the shock wave during this period. The injections corresponded to different HXR pulses and type III radio bursts, while shock associated features such as type II radio emissions were also recorded.

% \begin{itemize}    
%     \item [\textbullet]
%     In this study, we found that the coronal shock wave was able to accelerate electrons to a wide range of energies observed as the strong anti-sunward first in-situ component recorded at \textit{SolO}. This was due to the strongly structured nature of the corona during this time. In such cases, the shock wave can interact with adjacent coronal magnetic fields in a near-perpendicular regime which facilitates efficient acceleration of electrons.  
% \end{itemize}

%However, provided the conditions such as the availability of a broad tail population of electrons (supra-thermal and non-thermal electrons), and high magnetic compression can accelerate a small portion of these electrons to relativistic energy ranges. However, due to the small loss-cone and pitch angle requirements of the incident electrons, this process is severely curtailed at high energies leading to a roll over of the power-law spectra observed in-situ.

% \begin{itemize}    
%     \item [\textbullet]
%     We found that the second, gradual in-situ component with low-anisotropy was accelerated by the shock wave in a diffusive regime similar to the protons. We proposed that the seed population for the DSA regime may be provided by the scattered electrons from the first phase or through a second-order Fermi process present upstream of the shock wave. In our study, we have emphasised the role of the SIR compression which plays a crucial role in trapping the particles within a narrow region between the shock wave and the SIR compression.
% \end{itemize}

%This led to the second in-situ component being observed only by \textit{SolO}.  

% \begin{itemize}    
%     \item [\textbullet]
%     The low anisotropy of the second, gradual in-situ component is most likely due to the extended acceleration away from the source of the electrons. The second order Fermi acceleration of the electrons together with their release in a DSA regime could lead to the loss of the original directivity.  
% \end{itemize}

% \begin{itemize}    
%     \item [\textbullet]
%     Our study has found that the effects of interplanetary transport played a role for the particles arriving in \textit{STEREO-A}. Eventhough the magnetic field line connectivity between \textit{SolO} and \textit{STEREO-A} were close, they recorded the electron event significantly different. Based on the heliospheric conditions presented in \cite{Lario22} study of the same event, we found that this is the case because \textit{SolO} was located within the fast wind and therefore observed less transport effects maintaining the two phase structure. 
% \end{itemize}

% subdued when the observer is located in a region which confine the particles within a small regions e.g., SIR. The observers located outside these confined regions may record particles which are affected by interplanetary transport. In our study, the event observed by \textit{STEREO-A} which was located only 25$^{\circ}$ east of \textit{SolO} longitudinally was considerably different. We found that the electrons recorded at \textit{STEREO-A} did not have the "two" components which were observed by \textit{SolO}. The particles recorded by \textit{STEREO-A} were most likely associated with the high energy counterpart of the first component and had parts of the second component as well.


%We found that there was a first release of low-energy electrons followed by a second release of high-energy electrons several minutes later.

%Features relating to both flares, and shocks were observed during the first phase which suggests a complex relationship between the in-situ components and their solar acceleration mechanisms.
%The remote-sensing correspondence to the in-situ observations for both low and high energy electron injections, suggests a complex association with the different physical processes observed. 



%There may exist several acceleration mechanisms which could have played a role in the energization of both the low- and high-energy electrons during this phase leading to the first in-situ component. In the below subsections, we discuss briefly the different possible scenarios for electron acceleration and release during phase 1.
%During the inferred time of injection of the energetic electrons during the first phase, a wide variety of features in multiple wavelengths signifying different physical processes, namely, injection, trapping, and propagation of energetic electrons were observed in the corona. Since t

%The release of the low-energy electrons was accompanied by different physical features such as multiple HXR pulses (and the associated microwave emission), the first type III radio burst group (TIII-G1), and finally the start of the first type II radio burst (TII(1)). The inferred release of energetic electrons with energies higher than roughly 100 keV indicate that they were were clearly delayed compared to the start of the first type III radio burst \citep[e.g.][]{Kouloumvakos2015}. This inferred release time of the high-energy electrons corresponds to the second group of type III radio bursts (TIII-G2), the herringbone-type II (TII(HB)), the second type II (TII(2a)), and the type IV continuum. While the initial releases of the low and high-energy electrons at the Sun were separated by $\approx$ 5 \-- 10 minutes, the peak intensity of the electrons accelerated during the first phase was recorded considerably later at 06:52 UT (Fig. \ref{fig:timeline}). 


%When the magnetic compression (ratio between upstream and downstream magnetic field strength) at the expanding shock front is $\sim 3$ (can be $\sim 4$ for impulsive events), electrons with pitch-angle $\geq$60$^{\circ}$ ($\geq$70$^{\circ}$ for a magnetic compression ratio of $\sim 4$) can be readily accelerated to a wide range of energies at the loss of their incident pitch-angles.

%Provided that the electron density in the low corona is high ($10^9$~cm$^{-3}$ based on a 5-fold \cite{Newkirk61} coronal electron density model)
%\cite{Kong16} suggested that a shock wave expanding through coronal structures (e.g. Streamers, coronal holes, etc.,) is an efficient accelerator of electrons and would naturally produce a power-law-like energy spectrum.
%A low intensity for electrons with the highest energy gain (high pitch angles, > 70$^{\circ}$) and a high intensity for electrons with the lowest energy gain (low pitch angles, $\geq$60$^{\circ}$ \-- $\geq$70$^{\circ}$), which is power-law like with a hard-soft spectral index. 


%An interesting aspect of this phase was that the electron beams generating TIII-G2 could have interacted with the shock wave and have gotten re-accelerated. Based on the interplanetary directivity analysis of TIII-G2, we show that the source of the electron beams was well connected to both \textit{SolO} and \textit{STEREO-A} (Fig. \ref{fig:space_obs_all}). Therefore it is highly possible that the shock wave interacted with the source of TIII-G2. Such an interaction could have accelerated the incident low-energy flare accelerated electrons to far higher energies based on their incident pitch angles. Electrons with large enough pitch angles are readily reflected by a near-perpendicular shock wave gaining maximum energy of nearly 13-fold their initial energy in the process \citep[][]{Leroy84, Street94, Ball2001}. Such an efficient mechanism can increase the energy of a fraction (depends on $\theta_{Bn}$) of the incident $c/3$ electrons (generating TIII-G2) to near-relativistic energies. Considering that electrons in the range of 50 \-- 100 keV were also abundant in the flaring region, they were most likely released along with the $c/3$ electrons generating TIII-G2. These electrons can be further accelerated to relativistic energies on interaction with the coronal shock wave thereby, providing a compelling scenario for shock acceleration during this period. The TIV continuum observed during the same period was probably generated by electrons trapped within the flux rope of the expanding CME \-- some of these energised particles may have escaped during possible interactions between the CME and the ambient magnetic field lines. In such a case, the CME could have facilitated the release of some of the energetic electrons trapped within the closed loops of the CME \citep[][]{Petrosian16}. The released energetic electrons may have then interacted with the shock wave and in the process, accelerated further. An additional evidence for a shock acceleration scenario was the observations from the Suprathermal Ion Spectrograph (SIS) on-board \textit{SolO}. SIS showed no particular enhancement of flare accelerating particles such as $^3$He ions that would suggest a direct contribution of flare accelerated particles to the particle population measured in-situ during the event.

%An interesting aspect of this phase was that the electron beams generating TIII-G2 could have interacted with the shock wave and have gotten re-accelerated before their release to the two spacecraft. 
%An interesting aspect of this period was the possible interaction between the electron beams generating the TIII-G2 and the shock wave leading to re-acceleration of the incident electrons.

%\subsubsection*{Scenario 2: CIR mirroring}

%Nicolas and Nina can you please fix this section and write whatever that may be needed? 

%If we were to assume a completely exclusive scenario ignoring the presence of the interplanetary shock wave and its ability to accelerate electrons, which is dependent on a large variety of factors, we may do so by considering the presence of the stream/co-rotating interaction region (S/CIR). Stream interaction regions (SIR) and co-rotating interactions regions (CIR) are formed when faster solar wind interacts and piles up behind the slower wind giving rise to a shocked compression region \citep[][]{Pizzo78, Gosling96}. Due to this, energetic particles can be trapped within the compression region for extended periods of time \citep[][]{McComas19}. 

%Magnetic field line meandering is a well documented feature of the heliospheric plasma \citep[][]{Jokipii66, Jokipii69}. The effects of meandering magnetic field lines on particle transport is that, the often considered solution for the length of the Parker spiral would be erroneous. These transport effects in particular affect higher energy particles whose mean free path is far smaller than that of the low energy particles. 

%In this scenario, we consider part of the energetic electrons released during the first phase (discussed in Sec. \ref{subsec:phase_1} to have encountered meandering magnetic field lines \citep[][]{Jokipii66, Jokipii69} where the plasma outflow from both the nearby streamer and coronal holes interacted forming an CIR. The electrons can then be mirrored within the CIR by the compression region which would have the same effect as a fast-Fermi electron mirroring at a coronal shock wave dis

%Flare+shock acceleration?

%CIR reflection


%Perhaps we dont want to write too much about the Karlicky idea of the dM spikes

%We also note the drifting spike-like bursts starting at 1400 MHz around the start time of the flare at ~06:28 UT. The spike-like bursts form a rather broadband continuum in the decimeter-meter frequency range but are not observed below 200 MHz. \cite{Kliem00, Karlicky02, Karlicky04a} have suggested that they are signatures of electrons accelerated at the cusp of the reconnection point and are associated with the formation of plasmoids along a pre-existing current sheet. Another explanation provided by \cite{Aurass02a, Karlicky03Review,Karlicky04a, Mann09} was that they could be signatures of the reconnection process and the formation of a termination shock. The drift speed of the spike-like continuum would then indicate the speed of the reconnection process. Further analysis of this feature is presently beyond the scope of the current study and will be explored in a future study of the decimetric and metric radio observations from this event. 

%A second, relatively more intense type II burst was observed starting at a frequency of 450~MHz ($\approx$ 225 MHz for $f_{pe}$) at about 06:35:30~UT. In stark contrast with the first type II burst, it is the harmonic lane which exhibits intense emission. However, the type II is rather patchy and has markedly very little to no emission between 80 MHz and 50 MHz. The type II is brightened again at 50 MHz and lasts for 6 mins between 06:49~UT and 06:55~UT. During this period, the type II is observed with both a fundamental and harmonic lane. It also exhibits clearly distinguishable band splitting and comes to a cessation at 40 MHz ($\approx$ 20 MHz for $f_{pe}$).

%two separate type II radio bursts and multiple groups of type III radio bursts among other fainter type III bursts. The first type II radio burst is observed rather well and is somewhat continuous although lacking a clear backbone feature. The first type II exhibits clear fundamental and harmonic emission structure and also band splitting. The second type II on the other hand is brighter than the first and also appears to have a clear backbone feature while exhibiting both fundamental and harmonic emission and also band splitting. 

%It is often difficult to find type III bursts below 500 MHz due to absorption by inverse Bremsstrahlung \citep[][]{Melrose80, Reid14Review}, and so type III bursts in the 1 GHz range are usually considered to be harmonic emission. Keeping this in mind, we distinguish several fast drifting (almost instantaneous) emissions that correspond to the presence of energetic electrons in a beam-like distribution in the vicinity of the flaring region. Some of the electron beams that escape the flaring region can be observed as groups of type III radio bursts. This suggests the presence of open field lines leading away from the flaring active region for the streaming electrons to escape.

%Rarely, during solar flares the type III bursts can start in microwave frequencies rather than the typical 100-10 MHz range or even lower. While it is not a trivial task to distinguish between the F- and H- components, it is generally accepted that fundamental emission above 500 MHz is subject to severe absorption due to inverse Bremstrahlung radiation (Reidreview14). The presence of coulomb collisions also damps both electron and plasma waves and therefore making it difficult to generate radio emission. However, regions of high densities and regions which produce a large number of intense electron beams which can drive beam-plasma instabilities can generate radio emission.

%The brightening, which is most likely a result of the interaction between the shock wave (type II source) and the electron beam (type III source), was observed together with herringbone-like features. The observation of herringbone-like features suggests that the brightening may not merely be a projection of the type II and type III on the spectrum, but rather a physical interaction between the two sources in the decametric plasma. The presence of herringbone features may also imply re-acceleration of the energetic electrons by the shock wave. 

%and was most likely brightened as a result of the interaction between the shock wave and the electron beam.

%During the same time period, observations in the 1 GHz to 500 MHz show several type III radio bursts which suggest escaping non-thermal electrons through the open and quasi-open magnetic field lines. The two main groups (comprised of several type III bursts) are observed at 06:31, and 06:39 respectively.

%%The below text can be used as a concluding remark about the high energy injection..

%Such constraints fit the nature of our event as we suppose that the acceleration happens at low coronal heights and the seed population of electrons are supra-thermal or non-thermal in nature. The presence of quasi-perpendicular and near-perpendicular geometry is also confirmed by TII(HB), and TII(W) (Sec. \ref{subSec:Radio}). Incidentally, the intensity of high energy electrons observed in-situ were also low and peaked during the first phase of the event. The sustained increase in high energy electron flux during the second phase of the event is most likely due to an additional mechanism (discussed further in Sec. \ref{subsec:phase_2}.

%Lastly,  also serves as a possible candidate for electron acceleration \citep[][]{Matamoros16, Klein22}. 

%Type IV continuum emissions have therefore been associated with energetic electron events \citep[][]{Pick08, Aurass03}. \cite{Dresing21} have also suggested it to be a possible mechanism for delayed injections and also for their more wide-spread nature. However, their study also concluded that the CMEs themselves may not be responsible for accelerating near-relativistic or higher energy electrons. While they may not be able to accelerate electrons to relativistic energies, they could still release the electrons trapped within closed magnetic field lines in a wide angle \citep[][]{Reames13}. This adds further complexity to the origin of the electrons with energy greater than 80 keV.

%the mean free path of higher energy electrons is far smaller than that of the low-energy electrons and therefore, their  is far higher than that of low-energy electrons (Sanahuja ref?, Nicolas' modelling studies too probably? REF).

%During the reorganisation of magnetic field lines near the flaring region that is observed around the 3rd HXR peak any release of energetic electrons  may also release electrons in the 100 keV range. These electrons may not be radiating as type III radio bursts due to their low beam densities \citep[slow growth of beam instability;][]{Reid14Review} but could have propagated along the same open field lines as the ones generating TIII-G2. However, such energies are still far below the 1\,-- \,2~MeV energies of relativistic electrons which were also released during the same interval.

%Street and Melrose 1994 also suggest that the resultant spectra from a SDA accelerated electron component would be impulsive but lack the continued flux as observed in DSA. 

%The high energy component was observed by \textit{SolO} and \textit{STEREO-A} and were roughly 10 minutes apart based on TSA. Such a difference in the inferred injection time indicates that the high energy electrons were injected over an extended period beyond the TIII-G2 and TII(HB). The most relevant features during this time, at $\approx$ 06:47~UT were the 5th HXR peak, IP-TII(1), TII(2), TII(W), and finally the type IV continuum. While it is entirely possible that the continuous TII(1) could have been the accelerator, we shall also consider the EUV wave reflection at the coronal hole boundary at $\approx$ 06:50~UT (Sec. \ref{subSec:Shockwave}). During an after the reflection, TII(W) was observed and exhibits a similar spectral morphology to TII(HB). The emission also exhibited a "backbone" which would suggest a shock geometry that is not as perpendicular as the one generating TII(HB). However, the potential for electron acceleration remains albeit to a lower efficiency in terms of achievable kinetic energies. 

%Supercritical interplanetary oblique shock waves have therefore been observed to accelerate mildly-relativistic and relativistic electrons \citep[][]{Wilson12}. 

%comes down to its efficiency at accelerating and reflecting energetic ions which can then resonantly generate waves upstream of the shock at the ion cyclotron resonance frequency \citep[][]{Kennel81, Treumann08para}

%Patchy type II radio emissions such as the hectometer TII(2) are naturally generated in regions where the electron acceleration is most efficient in an oblique shock wave \citep[][]{Mann95c, Jebaraj21}.   

%It is therefore necessary to include the effects of upstream magnetic turbulence to get a wholesome picture of electron acceleration as the electrons in such environments can show a substantial variations of flux. 

%This process can continue as long as the amplitude of the magnetic perturbation or the direction of the magnetic field do not deviate far from the average amplitudes or directions.  

%Patchy type II radio emission such as TII(2) are great indicators of both shock deformation and upstream turbulence \citep[][]{Mann95c, Bemporad13}. Ambient ion-scale magnetic turbulence may provide efficient magnetic traps for electrons in a wide range of pitch-angles which can then gain substantial energies in a pitch-angle diffusion process \citep[][]{Giacalone05}. There is a strong possibility of this process in highly structured solar wind originating in regions close to the equatorial latitudes \citep[][]{Bale19}. Electrons in these regions can be reflected back and forth in a turbulent magnetic field \citep[within the probability distribution of ambient solar wind magnetic turbulence;][]{Yordanova09,ChenC13} along its average direction. This process can continue as long as the amplitude of the magnetic perturbation or the direction of the magnetic field do not deviate far from the average amplitudes or directions. For regions with high levels of turbulence, as the ones present in a magnetic compression, the electrons within the range of the accepted pitch-angles can remain trapped. 

%Inhomogeneity in the solar wind can also influence shock's morphology and its parameters on both spatial and temporal scale \citep[e.g.,][]{Florinski06, Giacalone07, Guo10, Senanayake13, Guo21}. The WL shock wave presented in Sec. \ref{subSec:Shockwave}) showed a strong propagation in the direction of the solar equatorial. These regions may diverge from a thermal Maxwellian electron population which is often assumed in the corona \citep[][]{Maksimovic97}. The suprathermal/non-thermal electrons can be mirrored off the shock wave and be trapped between the shock wave and the pre-existing upstream turbulence. \citep[][]{Yang18} found nearly 40 keV electrons trapped in the vicinity of an interplanetary shock wave at 1 AU with nominal magnetic field turbulence. The energy gained by the electrons trapped in the aforementioned conditions overtime can be in the order of 100s of keV for higher levels of magnetic turbulence \citep{Guo15}. It is therefore necessary to include the effects of upstream magnetic turbulence to get a wholesome picture of electron acceleration as the electrons in such environments can show a substantial variations of flux. 

%The presence of a suprathermal tail population in dynamic regions with magnetic fluctuations can provide the initial seed population for a DSA based acceleration. 

%The conditions may alternate significantly between quasi-parallel and quasi-perpendicular \citep[][]{Guo21}. 

%\citep[][]{Burgess06} found that the resultant energy spectrum from such a diffusive acceleration was ....

%Supercritical interplanetary oblique shock waves have been observed to accelerate mildly-relativistic and relativistic electrons \citep[][]{Wilson12}. Several numerical particle-in-cell (PIC) studies \citep[e.g.,][]{Amano10, Park12} have also considered the generation of whistler waves \citep[][]{Riquelme11} to be an important factor for accelerating non-relativistic and near-relativistic electrons to even higher energies. The self-generation of ion whistler waves by a supercrictical oblique shock primarily comes down to its efficiency at accelerating and reflecting energetic ions which can then resonantly generate waves upstream of the shock at the ion cyclotron resonance frequency \citep[][]{Kennel81, Treumann08para}. The acceleration in such a turbulent regime is strongly dependent on the characteristics of the upstream waves, namely, their amplitudes and damping time scale. It should be noted that, the process also is dependent on the characteristics of the trapped electrons such as their pitch-angles and initial energy \citep[][]{Bell78}. 


%Such a confined region if rippled will inherently act as a hot spot for accelerated electrons \citep[][]{Kong17}.

%This is due to the fact that the perpendicular diffusion is rather small compared to that of the parallel diffusion. Therefore, these regions of magnetic convergence then become "hot-spots" for accelerated electrons while regions further apart from the convergence zones are far less efficient at accelerating electrons. 

%Further evidence of such a near-perpendicular geometry is the absence of the backbone feature (as is the case with TII(HB)) which is usually observed in type II radio bursts \citep[][]{Kundu65, Melrose80}. This reinforces the fact that shock waves with a perpendicular ($\theta_{Bn} = 90^{\circ}$) geometry do not emit radio emission as they transmit all incident upstream electrons to the downstream regardless of incident energy or pitch angles \citep[][]{Ball2001}. TII(W) emission on the other hand exhibited a backbone and herringbones together. Such a morphology indicates a shock geometry that is not as perpendicular as the one generating TII(HB). In this case, the potential for electron acceleration remains, albeit a wider range of energies are to be expected as the loss-cone has a larger angle allowing electrons with lower pitch-angles to be accelerated \citep[][]{KraussV1989b}. 

%they do not particularly provide clues to whether electron above 80 keV could manifest as these type III radio bursts

%Furthermore, the presence of decimetric spike-like emissions (discussed in Sec. \ref{subSec:Radio}) indicates the presence of a possible flare related acceleration and release process \citep[][]{Alissandrakis88, Aschwanden85}.

% Type II radio bursts are generated by electrons accelerated in a scatter-free fast-Fermi process \citep[][]{Wu84}, and therefore the energy gain in such a scenario is limited \citep[but enough for Langmuir wave instability;][]{Mann22a}. However, the reflected electrons can arrive back at the shock, undergo multiple interactions and gain far higher energies \citep[][]{Leroy84}. Type II radio bursts can therefore provide vital information on the potential source regions or "hot spots" for electron acceleration.

%may  have found that multiple injections during the duration of the HXR flare is a possibility, however, there may exist an additional mechanism which is needed to describe the delays in acceleration. An additional mechanism involved in the acceleration of electrons may cause them to be observed at a wide longitudinal range. Further effects due to magnetic field turbulence would mean that they may have to undergo field line diffusion which may also reduce their level of anisotropy \citep[][]{Reames13}.

%SDA can also accelerate electron populations in a power-law tail depending on their pitch angles to even higher energies \citep[][]{Toptygin80, Ball2001}. 

%Given the observational data, the additional flux and the injection time of the low-energy electrons in the range 40-80 keV seems to fit rather well with the time of TII(1). 

%Shock curvature in corona is greater than the closed B field lines and therefore the flanks provide the best acceleration for electrons and can accelerate to energies exceeding 40 keV (Kong16)

%Propagating electron beams are seldom mono-energetic but are rather a distribution of different energies \citep[][]{Mann22b} and therefore different parts of the beam distribution are responsible for the generation of type III radio emissions at different heights. The nominal speed of electrons generating decametric type III radio bursts is considered to be $c/3$ ($\approx$ 25 keV; Lin et al. paper reference from their RHESSI+radio study, Sam Kruckers papers...). 

%Given the right conditions, faster electron beams can also generate variations of type III radio bursts, namely the type IIIn and type IIId bursts \citep[][]{Klassen03}. However, our observations do not show type III bursts with the type IIIn or type IIId spectral morphology, meaning that considering nominal $c/3$ speeds for TIII-G2 should be acceptable.

%%% abstract draft - taken from SolO8 abstract %%%
%We study the solar energetic particle (SEP) event observed on October 9, 2021, by multiple spacecraft including Solar Orbiter (SolO). The event was associated with an M3.7 flare, a coronal mass ejection (CME) and a shock wave. During the event, high-energy protons and electrons were recorded by multiple instruments located within a narrow longitudinal cone. An interesting aspect of the event was the multi-stage particle energization during the flare impulsive phase and also what appears to be a separate phase of electron acceleration detected at SolO after the flare maximum. 
 
%We utilize SEP electron observations from the Energetic Particle Detector (EPD) and hard X-ray (HXR) observations from the Spectrometer/Telescope for Imaging X-rays (STIX) on-board SolO, in combination with radio observations at a broad frequency range. We focus on establishing an association between the energetic electrons and the different HXR and radio emissions associated with the multiple acceleration episodes. 
 
%We will present our first results showing that the flare was able to accelerate electrons for at least 20 minutes during the non-thermal phase observed in the form of five discrete HXR pulses. We also show evidence pointing at the  possibility that the shock wave has contributed to the electron acceleration during and after the impulsive flare phase. The detailed analysis of EPD electron data shows that there was a time difference in the release of low- and high-energy electrons and also  that the electron anisotropy characteristics were different during the separate phases of electron energization.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%Maybe this information can be omitted or can go to the subsubsection where I describe S/C observations:
%Both instruments provide dynamic radio spectra and goniopolarimetric measurements at a number of discrete frequencies in the range 100--1046~kHz. The STEREO observations provide dynamic spectra in the range of 10--16000~kHz, and WIND in the range of 4--13825~kHz (three antennas cover the range of 4--256~kHz, 20-1040~kHz and 1075--13825~kHz). Goniopolarimetric observations at selected frequencies are provided in the similar frequency range for both spacecraft (100-1040~kHz), but the number of discrete frequencies is larger for the \textit{STEREO-A} spacecraft.
%We use observations from the Yamagawa radio observatory, and the Australia-ASSA e-callisto observatory

%probably because a type IV radio burst overlaps at the same time. 

%...and are usually considered to be signatures of flare associated blast waves or precursor emission of metric type II bursts. The precursor emission mainly consist of spike-like bursts drifting to lower frequencies %The diffuse and rather broadband nature of TII(2) suggests that it may be because it was observed together with the flare continuum and therefore was brightened due to this overlay. The type II was not observed after 06:45:30 UT around 150 MHz, which was close to the time and frequency below which the continuum stopped drifting. This further suggests that the type II burst may have been rather weak and was only enhanced due to the overlay of the continuum in the dynamic spectra.
% (shock rippling/oblique regions (SLAMS): Schmidt&Cairns 2012a,b, Mann+2022)
%the ongoing TII(1)

%This bright part of the type II emission exhibit clear herringbone structure (e.g. Morosan study in Nature)


%  The electrons in these regions can undergo a second-order Fermi acceleration, a process in which they undergo stochastic scattering in the turbulent magnetic field lines, gaining energy as a function of their pitch angles and the amplitude of the turbulent magnetic field along its average direction.  On the other hand, the shock wave can also be corrugated and develop small-scale features such as cavities and ripples at the front during its propagation through turbulent media \citep[e.g., stream interaction regions][]{Giacalone07, Yang12, Guo15}. Such small-scale features can be locally quasi-perpendicular or near-perpendicular leading to short and efficient acceleration of electrons trapped within them \citep[][]{Bale99}. Additionally, the self-generation of ion-scale whistler waves by a supercritical oblique shock wave are the most important factor for accelerating electrons to relativistic energies \citep[][]{Riquelme11}. A model which takes into account both upstream turbulence either induced by the shock wave or by a turbulent magnetic field was proposed by \cite{Katou19}. Their model assumes that both a first-order and second-order Fermi acceleration process can co-exist. In the stochastic shock drift acceleration (SSDA), the broadened tail distribution of electrons is provided by the second-order Fermi process which are then re-accelerated by a first-order Fermi process at the shock front.   

% A last aspect is that the patchy type II radio emissions such as hectrometric TII(2b) may be generated as natural consequences of an oblique shock wave expanding into electron rich structures \citep[][]{Jebaraj21}. \cite{Mann95c} have suggested that shock waves with oblique geometry can generate radio emission intermittently with high intensities such as those we observe in this event. The starting time and duration of TII(2b) indicates that the scenario we have presented here was present for a prolonged period. DSA is generally believed to produce gradual time-intensity profiles for accelerated particles. The observations suggest that during the second phase, a DSA-like mechanism was active where the high energy electrons may have resonantly gained energy from the waves generated by the protons accelerated during the same event. 
